Finite State Markov Modeling of C-V2X Erasure Links For Performance and Stability Analysis of Platooning Applications

Cooperative driving systems, such as platooning, rely on communication and information exchange to create situational awareness for each agent. Design and performance of control components are therefore tightly coupled with communication component performance. The information flow between vehicles can significantly affect the dynamics of a platoon. Therefore, both the performance and the stability of a platoon depend not only on the vehicle's controller but also on the information flow Topology (IFT). The IFT can cause limitations for certain platoon properties, i.e., stability and scalability. Cellular Vehicle-To-Everything (C-V2X) has emerged as one of the main communication technologies to support connected and automated vehicle applications. As a result of packet loss, wireless channels create random link interruption and changes in network topologies. In this paper, we model the communication links between vehicles with a first-order Markov model to capture the prevalent time correlations for each link. These models enable performance evaluation through better approximation of communication links during system design stages. Our approach is to use data from experiments to model the Inter-Packet Gap (IPG) using Markov chains and derive transition probability matrices for consecutive IPG states. Training data is collected from high fidelity simulations using models derived based on empirical data for a variety of different vehicle densities and communication rates. Utilizing the IPG models, we analyze the mean-square stability of a platoon of vehicles with the standard consensus protocol tuned for ideal communication and compare the degradation in performance for different scenarios.

==> control_stuff.tex <==
% The control stuff is simply added here for now and can be rearranged as suitable later
\section{Vehicle Modeling and Control}
\textcolor{red}{The control stuff is simply added in this section and should be rearranged wherever suitable later}

We consider a double integrator model governed by the dynamics, 
\begin{equation} \label{eqn:agent_dynamics}
\begin{split}
  \dot{x} &= v \\
  \dot{v} &= u.
\end{split}
\end{equation}
With a ZOH (Zero-Order-Hold) discretization with a sampling time $T$, the discrete-time dynamics can then be represented as
\begin{equation} \label{eqn:agent_dynamics_ZOH}
\begin{split}
  x_{k+1} &= x_{k} + T v_k + \frac{T^2}{2}u_k\\
  v_{k+1} &= v_k+T u_k.
\end{split}
\end{equation}
We consider the standard second order consensus protocol with reference position offset $r^{\textnormal{pos}}$ and reference velocity offset $r^{\textnormal{vel}}$ [Cite Fax and Murray or Olfati Saber]
\begin{equation} \label{eqn:consensus-protocol}
    u_k=K_p L(r^{\textnormal{pos}}_k-x_k)-K_dL(r^{\textnormal{vel}}_k-v_k),
\end{equation}
where $L$ is the Laplacian matrix [cite F.Bullo].
With state variable $z_k=[x_k \; v_k]^T$ and $r_k=[r^{\textnormal{pos}}_k \;
r^{\textnormal{vel}}_k]^T$, the closed loop dynamics can then be represented as
\begin{equation} \label{eqn:closed-loop MJLS}
z_{k+1}=A z_k+B r_k
\end{equation}
where,
\begin{equation}
\begin{split}
A&=\begin{bmatrix}
I-\frac{K_pT^2}{2}L & T I-\frac{K_dT^2}{2}L\\
-K_pTL & T I-K_dTL\\
\end{bmatrix}\\
B&=
\begin{bmatrix}
\frac{K_pT^2}{2}L & \frac{K_dT^2}{2}L\\
K_pTL & K_dTL\\
\end{bmatrix}
\end{split}
\end{equation}
We assume that the Laplacian matrix $L$ is a random process described by a Markov chain and sampled for each $k$ from a finite set $\mathcal{L}=\{ L_1,L_2,\cdots ,L_N \}$.
Since the matrices $A$ and $B$ are functions of $L$, these are random process as well sampled from appropriately defined sets $\mathcal{A}=\{ A_1,A_2,\cdots ,A_N \}$ and $\mathcal{B}=\{ B_1,B_2,\cdots ,B_N \}$. 
Let $T\in \mathbf{R}^{N \times N}$ denote the Transition Probability Matrix (TPM) for the underlying Markov chain such that for all $k$,  $T_{ij}=\textnormal{Prob}\{L_{k+1}=L_j|L_k=L_i\}$.
Dynamimcs \eqref{eqn:closed-loop MJLS} is then a Markovian Jump Linear System (MJLS) [cite Costa book].
For the MJLS \eqref{eqn:closed-loop MJLS}, define a matrix $\mathcal{S}=(T'\bigotimes I)\textnormal{blkdiag}(A_1,A_2,\cdots ,A_N)$
It has been shown [Cite costa book] that the dynamics \eqref{eqn:closed-loop MJLS} are mean square stable if and only if the spectral radius of $\mathcal{A}$ is less than 1.

